Tight bounds for counting colorings and connected edge sets parameterized by cutwidth

We study the fine-grained complexity of counting the number of colorings and connected spanning edge sets parameterized by the cutwidth and treewidth of the graph. While decompositions of small treewidth decompose the graph with small vertex separators, decompositions with small cutwidth decompose the graph with small \emph{edge} separators. Let $p,q \in \mathbb{N}$ such that $p$ is a prime and $q \geq 3$. - If $p$ divides $q-1$, there is a $(q-1)^{\text{ctw}}n^{O(1)}$ time algorithm for counting list $q$-colorings modulo $p$ of $n$-vertex graphs of cutwidth $\text{ctw}$ and for all $\varepsilon>0$ there is no algorithm running in time $(q-1-\varepsilon)^{\text{ctw}} n^{O(1)}$, assuming the Strong Exponential Time Hypothesis (SETH). - If $p$ does not divide $q-1$, there is a (folklore) $q^{\text{ctw}}n^{O(1)}$ time algorithm for counting list $q$-colorings modulo $p$ of $n$-vertex graphs of cutwidth $\text{ctw}$ and for all $\varepsilon>0$ there is no algorithm running in time $(q-\varepsilon)^{\text{ctw}} n^{O(1)}$, assuming SETH. The lower bounds are in stark contrast with the existing $2^{\text{ctw}}n^{O(1)}$ time algorithm to compute the chromatic number of a graph by Jansen and Nederlof~[Theor. Comput. Sci.'18]. Both our algorithms and lower bounds employ use of the matrix rank method, by relating the complexity of the problem to the rank of a certain `compatibility matrix' in a non-trivial way. We extend our lower bounds to counting connected spanning edge sets modulo $p$ and give an algorithm with matching running time for both treewidth and cutwidth.

==> img/Conclusion.tex <==
\section{Conclusion}

In this paper we give tight lower and upper bounds for counting the number of (list) $q$-colorings and connected spanning edge sets of graphs with a given cutwidth decomposition of small cutwidth.
%
Our results on modular counting the number of colorings show that the modulus can influence the complexity in interesting ways, and that in some cases this rank can be directly explained by the rank of the compatibility matrix. 
 
Our results leave several directions for further research:
\begin{itemize}
	\item What is the fine-grained complexity of evaluating other points of the Tutte polynomial (modulo $p$)?
	\item What is the complexity of counting homomorphisms to graphs different from complete graphs, e.g. cycles or paths. Is it still determined by the rank of an associated compatibility matrix?
\end{itemize}

Another question in the direction of fast \emph{decision problems} is how small representative sets we can get for the compatibility matrix of graphs other than complete bipartite graphs (which is equivalent to the setting of \cite[Theorem 1.2]{FominLPS16}) or matchings which has been studied for the decision version in~\cite{jansen2019computing}.



==> img/EdgesetUpperbound.tex <==
\section{Proof of Theorem \ref{thm:main_upperboundcse}, upper bound}
\label{sec:upperboundcse}
Let $p$ be a prime. In this section we show that there is an algorithm that counts the number of connected spanning edge sets modulo $p$ in an $n$-vertex graph of treewidth at most $\tw$ in time $p^{\tw}n^{O(1)}$. The algorithm uses dynamic programming on the tree decomposition, reminiscent of cut-and-count. We will first need some additional notions about tree decompositions.

Let $G$ be an $n$-vertex graph with a tree decomposition $(T,(B_x)_{x\in V(T)})$ such that $T$ is a rooted tree and $|B_x|\leq \tw+1$ for all $x\in V(T)$.  Since $T$ is rooted, we can consider the children and  descendants of $x$ in $T$.
In polynomial time, we can adjust the tree decomposition to an edge-introduce tree decomposition without increasing the width. For an  \emph{edge-introduce}  tree decomposition (called a nice tree decomposition in \cite{cygan2011solving}) all bags $B_x$ are of one of the following types:
\begin{itemize}
\item Leaf bag: $x$ is a leaf of $T$.
\item Introduce vertex bag: $x$ is an internal vertex of $T$ with a single child $y$ for which $B_x = B_y \cup \{v\}$ for some vertex $v\in V(G)\setminus B_y$.
\item Introduce edge bag: $x$ is an internal vertex of $T$ with a single child $y$ with $B_x=B_y$, and $x$ is moreover labelled by an edge $uv \in E(G)$ with $u,v\in B_y$. Every edge in $E$ is `introduced' (used as label) exactly once.
\item Forget bag: $x$ is an internal vertex of $T$ with a single child $y$ for which $B_x = B_y \setminus \{v\}$ for some $v\in B_y$.
\item Join bag: $x$ is an internal vertex of $T$ with two children $y$ and $z$ for which $B_x=B_y=B_z$.
\end{itemize} 
We write $G_x$ for the graph on the vertices in the bags that are a descendant of $x$ in $T$, which has as edge set those edges that have been `introduced' by some bag below $B_x$. 


\begin{proof}[Proof of Theorem \ref{thm:main_upperboundcse}]
By the discussion above, we assume that an edge-introduce tree decomposition $(T,(B_x)_{x\in V(T)})$ for $G$ has been given.
For each $x \in V(T)$ and each partition $X_1,\dots,X_p$ of $B_x$, we define
%\unsure{I: Should $\cup V_i = V(G_x)$?}
\begin{align*}
T_x[X_1,\dots,X_p] =|\{(X,V_1,\dots,V_p)\::\:& V_1\sqcup \dots \sqcup V_p= V(G_x),\\
												&X\subseteq E(G_x) \setminus (\cup_{i<j} E(V_i,V_j)) \}|,
\end{align*}
where $\sqcup$ denotes the disjoint union (that is, we take the union and assume the sets are disjoint).
Thus, we count the number of edge sets $X$ of $G_x$ and number of vertex partitions $P$ of $G_x$ such that $X$ does not `cross' $P$ and $P$ `induces' the partition $(X_1,\dots,X_p)$ on $B_x$. Note that this is not done modulo $p$, but over the reals, and also that we do not put in the `connected spanning' constraints.

We claim that for $r$ the root of $T$, 
\[
\frac1p \sum_{R_1,\dots,R_p} T_r[R_1,\dots,R_p]
\]
equals the number of connected spanning edge sets of $G$ modulo $p$, where the sum is over the possible partitions of $B_r$. Note that $\sum_{R_1,\dots,R_p} T_r[R_1,\dots,R_p]$ counts the number of tuples $(X,V_1,\dots,V_p)$ such that $X$ is an edge set of $G$ that does not cross the partition $(V_1,\dots,V_p)$.  For an edge set $X$ of $G$, let $U_1,\dots, U_k$ denote the connected components (which may be single vertices) of $G[X]$, the graph with vertex set $V(G)$ and edge set $X$. The number of partitions $(V_1,\dots,V_p)$ of $G$ for which $X$ respects the partition equals $p^k$: we assign each connected component an element of $[p]$. Therefore,  the contribution of each $X$ to $\sum_{R_1,\dots,R_p} T_r[R_1,\dots,R_p]$ is divisible by $p$, and is divisible by $p^2$ if and only if $G[X]$ is not connected. This proves the claim since $G[X]$ is connected if and only if $X$ is connected and spanning.

What remains to show is that we can calculate the table entries in the claimed time complexity. If $x \in V(T)$ is a leaf, then we can calculate the table entry naively. We now assume that all strict descendants of $x$ already have their table entry calculated. We consider two cases.

Suppose first that $B_x$ is a `join bag': $x$ has two children $y$ and $z$ with $B_x=B_y=B_z$, and $E(G_y)\cap E(G_y)=\emptyset$. For any partition $(X_1,\dots,X_p)$ of $B_x$, we can also consider this as a partition of the bags $B_y$ and $B_z$. We claim that
\[
T_x[X_1,\dots,X_p] = T_y[X_1,\dots,X_p]\cdot T_z[X_1,\dots,X_p].
\]
This follows from the fact that any $(V_1,\dots,V_p,X)$ counted for $T_x[X_1,\dots,X_p]$, is determined by the following parts: the partition $X_1,\dots,X_p$ of $B_x$ (which is `fixed'), the remaining partition of the vertices in 
\[
V(G_x)\setminus V(B_x)=(V(G_y)\setminus V(B_x))\sqcup (V(G_z)\setminus V(B_x))
\]
(where we obtain a disjoint union by the standard tree decomposition properties) and the edge set $X\subseteq E(G_x)=E(G_y)\sqcup E(G_z)$ (where we find a disjoint union by our additional `edge-introduce' property).

Suppose now that $x$ has a single child $y$. Fix a partition $P_x=(X_1,\dots,X_p)$ for $B_x$ and consider a partition $P_{y}=(Y_1,\dots,Y_p)$ of $B_y$ that agrees with the partition $P_x$, in the sense that $X_i\cap Y_j=\emptyset$ for $i\neq j$. Note that since $|B_y \setminus B_x|\leq 1$, there are at most $p$ partitions $P_y$ that agree with $P_x$. We can therefore efficiently compute 
\begin{equation}
\label{eq:cseupp}
C \sum_{P_{y}:P_{y}\sim P_x} T_{y}[Y_1,\dots,Y_p]
\end{equation}
where the sum is over those $P_{y}=(Y_1,\dots,Y_p)$ that agree with the partition $P_x=(X_1,\dots,X_p)$, and where $C=C(X_1,\dots,X_p,y)$ is given by the number of possible subsets of $E(G_x)\setminus E(G_{y})$ that respect the partition $P_x$ (always counting the empty set). We will now show that (\ref{eq:cseupp}) equals $T_x[X_1,\dots,X_p]$.

When we fix a partition $(V_1,\dots,V_p)$ of $V(G_x)$ agreeing with $P_x$, then this uniquely defines a partition $P_y$ agreeing with $P_x$, namely $Y_i=V_i\cap B_y$ for all $i\in [p]$. Similarly, any partition $(V'_1,\dots,V_p')$ of $V(G_y)$ agreeing with $P_y$ (for some $P_y$ agreeing with $P_x$), uniquely defines a partition $(V_1,\dots,V_p)$ of $V(G_x)$ that agrees with $P_x$ (where we may need to add a vertex from $B_x\setminus B_y$ in the place specified by $P_x$). 

If $x$ is not introducing an edge, then $E(G_x)=E(G_y)$. Therefore, there is a one-to-one correspondence between tuples $(V_1,\dots,V_p,X)$ counted for $T_x$ and tuples $(P_y,V_1\cap B_y,\dots,V_p\cap B_y,X)$ counted for  (\ref{eq:cseupp}). Since in this situation $C=1$,  (\ref{eq:cseupp}) indeed equals $T_x[X_1,\dots,X_p]$.

If $x$ is introducing the edge $uv\in E(G_x)\setminus E(G_y)$ and $uv$ respects the partition $P_x$, then there is a two-to-one correspondence between tuples $(V_1,\dots,V_p,X')$ and $(V_1,\dots,V_p,X'\cup \{uv\})$ counted for $T_x$ and tuples $(P_y,V_1\cap B_y,\dots,V_p\cap B_y,X')$ counted for  (\ref{eq:cseupp}), where $X'\subseteq E(G_y)$. In this case $C=2$. If $uv$ does not respect the partition, there is a one-to-one correspondence again and $C=1$. This proves that  (\ref{eq:cseupp}) equals $T_x[X_1,\dots,X_p]$ in all cases.

The number of partitions $(X_1,\dots,X_p)$ of a bag $B_x$ is at most $p^{|B_x|}$ (assign each vertex of $B$ to an element of $[p]$). The computation of a single table entry is always done in time polynomial in $n$, and the size of the tree is also polynomial in $n$. Therefore, the running time of this algorithm is at most $p^{\tw}n^{O(1)}$.
\end{proof}
